Distributed Deep Joint Source-Channel Coding over a Multiple Access Channel

We consider distributed image transmission over a noisy multiple access channel (MAC) using deep joint source-channel coding (DeepJSCC). It is known that Shannon's separation theorem holds when transmitting independent sources over a MAC in the asymptotic infinite block length regime. However, we are interested in the practical finite block length regime, in which case separate source and channel coding is known to be suboptimal. We introduce a novel joint image compression and transmission scheme, where the devices send their compressed image representations in a non-orthogonal manner. While non-orthogonal multiple access (NOMA) is known to achieve the capacity region, to the best of our knowledge, non-orthogonal joint source channel coding (JSCC) scheme for practical systems has not been studied before. Through extensive experiments, we show significant improvements in terms of the quality of the reconstructed images compared to orthogonal transmission employing current DeepJSCC approaches particularly for low bandwidth ratios. We publicly share source code to facilitate further research and reproducibility.

==> figures/nn_architecture.tex <==
\begin{table*}[!tp]
\centering
\caption{Detailed \gls{NN} architecture of the employed encoder and decoder}
\label{tab:nn_architecture}
\begingroup
\renewcommand{\arraystretch}{1.5} % Default value: 1
\begin{tabular}{lll}
\toprule
Component                & Layer                                   & Output Shape                     \\ \midrule
Encoder $i=1,2$ (at Tx1 and Tx2) & Input $\Tilde{\xv}_{i,t} = \begin{bmatrix} \xv_{i,t} & \rv_i \end{bmatrix}^T$                & $4 \times W \times H$            \\
                         & Residual Block Downsample ($s=2,N=256$) & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & AF Module                               & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & Residual Block ($N=256$)                & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & Residual Block ($N=256$)                & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & AF Module                               & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & Attention Module                        & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & AF Module                               & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & Residual Block ($N=256$)                & $256 \times \frac{W}{2} \times \frac{H}{2}$      \\
                         & Residual Block Downsample ($s=2,N=256$) & $256 \times W/4 \times H/4$      \\
                         & AF Module                               & $256 \times W/4 \times H/4$      \\
                         & Residual Block ($s=1,N=\frac{64k}{WH}$)       & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & AF Module                               & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Attention Module                        & $\frac{64k}{WH} \times W/4 \times H/4$ \\
%                         & Precoding                               & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Power Normalization                     & $\frac{64k}{WH} \times W/4 \times H/4$ \\ \midrule
\gls{MAC}                & Sum Pooling and Noise Addition          & $\frac{64k}{WH} \times W/4 \times H/4$ \\ \midrule
Decoder at Rx            & Attention Module                        & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & AF Module                               & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times W/4 \times H/4$ \\
                         & Residual Block Upsample ($s=2,N=256$)   & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & AF Module                               & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & AF Module                               & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & Residual Block ($N=256$)                & $\frac{64k}{WH} \times \frac{W}{2} \times \frac{H}{2}$ \\
                         & Residual Block Upsample ($s=2,N=6$)     & $6 \times W \times H$            \\
                         & AF Module                               & $6 \times W \times H$            \\
                         & Output Images $\begin{bmatrix} \hat{\vec{x}}_{1,t} & \hat{\vec{x}}_{2,t} \end{bmatrix}^T$ & $2 \times 3 \times W \times H$   \\ \bottomrule
\end{tabular}
\endgroup
\end{table*}

==> figures/tab_channel_conditions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[!tbp]
\caption{Comparison of methods in terms of wireless channel conditions for two-user case}
\label{tab:channel_conditions_comparison}
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
Method        & Noise Variance & Average Power per Bandwidth & Bandwidth per User & Total Power per User \\ \midrule
DeepJSCC-TDMA & $\sigma^2$ & $2\Pavg$                         & k/2                & $k\Pavg$                           \\
DeepJSCC-NOMA  & $\sigma^2$ & $\Pavg$                          & k                  & $k\Pavg$ \\
\bottomrule
\end{tabular}
\end{table*}

==> sections/journal_extension.tex <==
We calculate \gls{MS-SSIM} based image quality measure $Q_{\mathrm{\gls{MS-SSIM}}}$ as:
\begin{align}
\label{eq:mssim}
Q_{\mathrm{\gls{MS-SSIM}}} (\vec{x}, \hat{\vec{x}}) = [l_M(\vec{x}, \hat{\vec{x}})]^{\alpha_{M}}\prod_{j=1}^{M}[a_{j}(\vec{x}, \hat{\vec{x}})]^{\beta_{j}}[b_{j}(\vec{x}, \hat{\vec{x}})]^{\gamma_{j}},
\end{align}
where
\begin{align*}
  &l_M(\vec{x}, \hat{\vec{x}}) = \frac{2\mu_{x}\mu_{\hat{x}}+v_{1}}{\mu_{x}^{2}+\mu_{\hat{x}}^{2}+v_{1}}, \\
  &a_{j}(\vec{x}, \hat{\vec{x}}) = \frac{2\sigma_{x}\sigma_{\hat{x}}+v_{2}}{\sigma_{x}^{2}+\sigma_{\hat{x}}^{2}+v_{2}}, \\
  &b_{j}(\vec{x}, \hat{\vec{x}}) = \frac{\sigma_{x\hat{x}}+v_{3}}{\sigma_{x}\sigma_{\hat{x}}+v_{3}}.
\end{align*}
$\mu_\vec{x}$, $\sigma_\vec{x}$, $\sigma_{\vec{x}\hat{\vec{x}}}$ are the mean and variance of $\vec{x}$ and covariance between $\vec{x}$ and $\hat{\vec{x}}$ respectively. $v_{1}$, $v_{2}$ and $v_{3}$ are coefficients for numeric stability; $\alpha_{M}$, $\beta_{j}$, and $\gamma_{j}$ are the weights for each components, which we use default values by the original paper except {\bf TODO}~\cite{wang2003multiscale}. After calculating either~\eqref{eq:psnr} or~\eqref{eq:mssim} for every image in the dataset, we take average over the images in the dataset.
% TODO: advantage of mssim over psnr and sim
%The second metric to determine image reconstruction quality used in this paper is \gls{MS-SSIM}.
\gls{MS-SSIM} has been shown to perform better than \gls{PSNR} in terms of human perception. In the low bandwidth scenario, \gls{PSNR} metric tends to give more 'average' results to satisfy its condition; however, it may leads to bias. Secondly, in the semantic communication perspective, \gls{MS-SSIM} metric is widely accepted according to the aim of transmission.

